PAC-Learning for Strategic Classification

The study of strategic or adversarial manipulation of testing data to fool a classifier has attracted much recent attention. Most previous works have focused on two extreme situations where any testing data point either is completely adversarial or always equally prefers the positive label. In this paper, we generalize both of these through a unified framework for strategic classification, and introduce the notion of strategic VC-dimension (SVC) to capture the PAC-learnability in our general strategic setup. SVC provably generalizes the recent concept of adversarial VC-dimension (AVC) introduced by Cullina et al. arXiv:1806.01471. We instantiate our framework for the fundamental strategic linear classification problem. We fully characterize: (1) the statistical learnability of linear classifiers by pinning down its SVC; (2) its computational tractability by pinning down the complexity of the empirical risk minimization problem. Interestingly, the SVC of linear classifiers is always upper bounded by its standard VC-dimension. This characterization also strictly generalizes the AVC bound for linear classifiers in arXiv:1806.01471.

==> intro_jan27.tex <==
\section{Introduction}
\label{sec:intro}
In today's increasingly connected world, it is rare that an algorithm will act alone. When a machine  learning algorithm is used to make predictions or decisions about others who have their own preferences over the learning outcomes, \emph{gaming behaviors} may arise. This is certainly not a new observation, and has been well-known as the \emph{Goodhart's law}, which is why policy makers prefer to make
decision and classification rules confidential \cite{Citron201489WashLRev0001TS}.
However, this is not fool-proof  in general since the methods can be reverse engineered in many settings. Moreover, transparency of machine learning methods is sometimes mandated by law, e.g.,~\cite{goodman2016regulations}. 
Gaming behaviors have been observed in a variety of domains such as finance~\cite{gaming-loan}, online retailing \cite{hannak2014measuring},  
education \cite{hardt2016stratclass} as well as the recent COVID-19 pandemic \cite{unemploy-benefits,avoid-test}. Such concerns have raised significant recent interests in designing  learning algorithms that are robust to strategic gaming behaviors of the data sources \cite{Perote2004StrategyproofEF,dekel2010incentive,hardt2016stratclass,chen:ec18,dong:ec18,cullina:nips18,awasthi2019robustness}; the present work subscribes to this literature. %Perhaps the most widely studied two classes of problems are strategic classification and strategic regression \todo{cite here}. 
\anil{Some references like gam, une, avo look weird. We could insert the COVID example here.}

This paper focuses on the ubiquitous binary classification problem, and we look to design classification algorithms that are robust to gaming behaviors \emph{during the test phase}. We study a strict generalization of the canonical classification setup that naturally incorporates data points' \emph{preferences} over classification outcomes (which leads to strategic behaviors as we will describe later). In particular, each data point is denoted as a tuple $(\x, y, r)$ where $\x$ and $y \in \{ -1, +1 \}$ are the \emph{feature} and \emph{label}, respectively (as in classic classification problems), and additionally, $r \in \RR$ is a real number that describes how much this data point prefers label $+1$ over $-1$. Importantly, we allow $r$ to be negative, meaning that the data point may prefer label $-1$. Let  set $R \subseteq \RR$ denote the set of all possible values that the preference value $r$ may take. Obviously, the trivial singleton set $R = \{ 0 \}$ corresponds to the classic classification setup without any preferences. Another special case of $R = \{ 1 \}$ corresponds to the situation where all data points prefer label $+1$ equally. 
%\anil{the setup might be a bit hard to follow since the notion of manipulation is not yet defined. Might be easier to follow if the basic setup is first defined, then the generalization is described} 
This corresponds to the strategic classification settings studied in several previous works \cite{hardt2016stratclass,hu:fat19,miller2019strategic}. Our model considers \emph{general preference} set $R$. As we will prove, this much richer set of preferences may sometimes make learning more difficult, both statistically and computationally, though  not always. 

% \hf{not emphasizing much that issues happens during only the testing phase, also mention all papers we are citing is the same setup }


Similar to many works in this space \cite{hardt2016stratclass,dong:ec18,hu:fat19,milli:fat19}, our model assumes that manipulation is only possible to the data \emph{features} and happens only during the \emph{test} phase.  Specifically, the true feature of the test data may be altered by the  strategic data point. The cost of  masking a true data feature $\x$ to appear as a different feature $\z$ is captured by a \emph{cost function} $c(\z; \x)$. Therefore, 
%the decision faced by such a strategic data point is to mask his feature $\x$ to appear as $\z$ so that $\z$ induces the preferred label of this data point, depending on the sign of his $r$. The intricacy of 
the test data point's decision needs to balance the \emph{cost} of altering feature and the \emph{reward} of inducing his preferred label determined by $r$.   As is standard in game-theoretic analysis, the training data point is assumed a rational decision maker and will choose the optimal feature $\z$ to alter to. Importantly, the data point's strategic behaviors will \emph{not} change its true label; this is  referred to as the strategic \emph{gaming} behaviors. A relevant but crucially different type of strategic behavior is  strategic \emph{improvement}, which changes the data point's label or intrinsic qualities \cite{kleinberg2019classifiers,miller2019strategic}. We refer interested readers to \cite{miller2019strategic} for a in-depth discussion of the differences among these two types of behaviors.  

% \anil{it might be easier to follow if this setup is introduced a bit earlier} 
The classification procedure goes as follows: (1) the learner computes a classifier $h$ based on a set of \emph{unaltered  training data} $\{ (\x_i, y_i, r_i) \}_{i=1}^n$ drawn from distribution $\D$ independently; (2) the test data point $(\x, y, r)$, also drawn independently from $\D$, observes the classifier $h$ first, and strategically responds to $h$ by altering to  feature $\z$ that maximizes his quasi-linear utility $[r \cdot \II(h(\z) = 1) - c(\z; \x)]$. This gives rise to a natural \emph{Stackelberg game} between the learner (leader, she) and the test data point (follower, he). %\footnote{More precisely, this is known as the Bayesian Stackelberg game in the literature \cite{conitzer2006computing}  since the test data point is drawn from a distribution $\D$.} 
We thus adopt the standard solution concept of \emph{Stackelberg equilibrium}, and aim to find the optimal classifier $h^*$ for the learner that minimizes her 0-1 classification loss (equivalently, maximizes classification accuracy), assuming that any test data point sampled from $\D$ will respond strategically. Note that the strategic Stackelberg equilibrium (SSE) also includes the test data point's best-response manipulated feature $\z$ to $h^*$, which however will be easy to compute given $h^*$ in our setup.  
%\todo{maybe discuss motivations of knowing training data correctly. } 

The above strategic classification model is natural and well-motivated. In fact, restricted \emph{special cases} of this  model have been considered in previous works \cite{bruckner2011stackelberg,hardt2016stratclass,cullina:nips18}, among which two of them are most relevant to ours. The first is   the seminal work on strategic classification by Hardt et al. \cite{hardt2016stratclass}. They considered a special case of our model where  each test data point always, and equally, prefers label $+1$. This corresponds to our model with a special preference set $R = \{1 \}$.   Our setup allows general preference set $R$ and  can model \emph{heterogeneous} preferences  among  data points. This largely enriches the possible strategic behaviors that can be captured by our setup. Besides motivating domains such as spam filtering and university admission  considered in previous works \cite{bruckner2011stackelberg,hardt2016stratclass}, a notable application domain that falls into our generalized setup, but not previous models, is the use of classification implemented by decision rules to determine who to take virus tests at the early stage of a pandemic (see. e.g., the CDC's rule for selected COVID-19 testing \cite{covid-test-rule}). In this situations, different people have different preferences of getting tests or not. Specifically, those with jobs that are easily adaptable to working from home prefer to get tested in order to know their true health status whereas those who have lower income, or do not get paid when quarantining at home, or cannot easily adapt to working from home would prefer to not get tested since a positive testing outcome may cause them to lose jobs and income \cite{avoid-test}. % Strategic response to the policy maker's classification  of selecting potential virus carriers for testing have been observed during COVID-19 pandemic \todo{cite here}. \anil{if we don't find concrete citations to this, should we tone this down?}

The second line of works most relevant to ours is classification under evasion attacks \cite{biggio:ecml13,goodfellow2015explaining,li2014feature,cullina:nips18,awasthi2019robustness}.   Here also training data are assumed uncontaminated whereas each test data point $(\x, y)$ can alter its feature vector  within an allowable region  to induce a classification label \emph{opposite} to its true label $y$, i.e., the ``adversarial'' assumption. This turns out to be another special case of our model with $r = -y \in \{ -1, 1 \} = R$ for each test data point %(i.e., the data point adversarially prefers the opposite of its true label) 
and the cost function is defined as $0$ in the allowable moving region and $\infty$ otherwise. In a recent intriguing work, Cullina et al. \cite{cullina:nips18} considered the question of probably approximately correct (PAC) learning for this classification problem with evasion attacks. They introduced the notion of adversarial VC-dimension (AVC) and proves that AVC is at most $d+1$ for linear classifiers when the feature vector $\x \in \RR^d$. In this paper, we strictly generalize the AVC to our strategic setup, which we coin \emph{strategic VC-dimension} (SVC). We study properties of SVC, its relation to AVC, and characterize SVC for linear classifiers. Notably, we show that AVC is  equivalent to SVC for the special preference set $R=\{-1, 1\}$, but with a general preference set $R$, SVC can be arbitrarily larger than AVC due to much richer class of strategic manipulations. Next, we elaborate our results in more details.  
\anil{The above two paragraphs are discussed in some form in section 1.2. One possibility is to cut these into a couple of lines-- just say that the work of Hardt and Cullina is relevant and put a forward pointer. Also, should we move the COVID example into the first paragraph of intro?}

\subsection{Our Contributions}
\todo{add a table to summarize}
\fan{\begin{enumerate}
    \item First, we establish the PAC-learning result under the general strategic setting by introducing a novel notion of \emph{strategic VC-dimension} (SVC), which generalizes the concept of adversarial VC-dimension (AVC) introduced by \cite{cullina:nips18}. We recover the learnability result for linear classifiers from \cite{cullina:nips18} by showing SVC=AVC in that particular setting and also show SVC can be arbitrarily larger than both AVC and the standard VC dimension in general.
    \item We also provide computational learnability result for linear classifiers. We point out that the empirical risk minimization problem is solvable when and only when the allowed strategic behavior pattern exhibits certain adversarial nature. 
    \item Finally, we study the power and limits of randomization in strategic classification. Surprisingly, we find that randomization may strictly increase the accuracy in general, but does not help in the special case of adversarial classification under evasion attacks. (actually, why it is the case? I though we only proved Randomization does not help in any perfectly separable adversarial classification problems.)
\end{enumerate}}
\noindent{\bf The Strategic VC-Dimension.} To capture fully general heterogeneous data preferences, we  introduce the novel notion of \emph{strategic VC-dimension} SVC($\H, R, c$) which naturally captures the complexity of any hypothesis class $\H$ in strategic classification setups when test data points' strategic behaviors are induced by cost function $c$ and preference values from set $R \subseteq \RR$. We show that any strategic classification problem is agnostic PAC learnable by the empirical risk minimization paradigm with  $O \big( \epsilon^{-2}[d \log(\frac{d}{\epsilon}) + \log(\frac{1}{\delta}))] \big)$ samples, where $d=$SVC($\H, R, c$) is the SVC.  Conceptually,  this result illustrates that SVC correctly characterizes the learnability  of the hypothesis class $\H$ in our strategic setup. 
%As mentioned earlier, our strategic classification model generalizes the adversarial classification model of Cullina et al. \cite{cullina:nips18}. Indeed, 
We formally show that our SVC notion strictly generalizes the adversarial VC-dimension (AVC) introduced in \cite{cullina:nips18} for adversarial learning with evasion attacks. Specifically, we prove that AVC equals precisely SVC($\H, R, c$) for $R=\{-1,1 \}$ when  data points' allowable moves are within region  $\{ \z; c(\z;\x) \leq 1 \}$ in AVC. %Therefore, AVC can be viewed as SVC under restrictive  preference set $R = \{ -1, 1 \}$ for data points. 
However,  for general preference set $R$, SVC can be arbitrarily larger than both AVC and the standard VC dimension. This illustrates that complex strategic behaviors can indeed make the learning statistically  more difficult. Interestingly,  to our knowledge, this is the first time  that adversarial learning and strategic learning are studied under the same framework. 

% \anil{might be useful to give a big picture summary about the different aspects of cost functions we consider, including asymmetric. Is it useful to mention contast with Hardt and separable functions here?}
\noindent {\bf Implication of SVC in Strategic Linear Classification. Efficient Statistical Learnability:}  Next, we consider strategic classification for the widely adopted hypothesis class, \emph{linear classifiers}. Here, features are in $\RR^d$ linear space and the cost function $c(\z;\x)$ for any $\x$ is assumed to be induced by arbitrary seminorms of the difference $\z - \x$. We distinguish between two situations which turn out to significantly affect the efficiency of learning: (1) \emph{instance-invariant} cost function which means the cost of altering the feature $\x$ to $\x + \Delta$ is the same for any $\x$; (2) \emph{instance-wise} cost function which allows the cost from $\x$ to $\x + \Delta$ to be different for different $\x$ (note that the separable cost function considered by Hardt et al.~\cite{hardt2016stratclass} is an instance-wise cost function). Our results illustrate sharp contrast --- in terms of both statistical learnability and computational tractability --- between these two situations. In particular, the SVC of linear classifiers is shown to be $\infty$ for \emph{instance-wise} cost functions even when features are in $\RR^2$ whereas the SVC is at most $d+1$ for \emph{instance-independent} cost functions where  features are in $\RR^d$. This later result also strictly generalizes the AVC bound for linear classifiers proved in \cite{cullina:nips18}, and illustrates the following interesting conceptual message: though SVC can be significantly larger than AVC in general,  \emph{extending from $R = \{ -1, 1\}$ (the adversarial learning setting) to an arbitrary preference set $R$ (which corresponds to strategic learning) does not increase the strategic VC-dimension of linear classifiers}.  
% Therefore, in linear classification, 
\noindent {\bf Efficient Computational Learnability. } On the computational side, we prove that the empirical risk minimization problem for linear classifier can  be solved in polynomial time when the strategic classification problem exhibits certain \emph{adversarial} nature. In particular, we say the instance has \emph{generally adversarial} preferences if all negative test points prefer label $+1$ (but possibly to different extents) and all positive test points prefer label $-1$.   A strictly relaxed situation has  \emph{essentially adversarial} references; that is, any negative test point prefers label $+1$ more than any positive test point.\footnote{This is a strict generalization of generally adversarial preferences since positive points may also prefer label $+1$ in this case, but not as much as negative points.} We show that for instance-invariant cost functions, any essentially adversarial instance can be solved in polynomial time whereas for instance-wise cost functions, only generally adversarial instances can be solved in polynomial time. Moreover, we prove that these positive results are essentially the best one can hope for. Formally, the following situations, which goes slightly beyond the tractable situations above, are both NP-hard: (1) instance-invariant cost functions but general preferences; (2) instance-wise cost functions but essentially adversarial preferences. 
\anil{we bring up the comparison with Hardt and Cullina in this subsection itself. So there is some duplication with the text in section 1.2}

Finally, we  examine the power and limits of \emph{randomization} in strategic classification. It is well-known that randomization does not improve classification accuracy in non-strategic settings (see, e.g., \cite{braverman2020role}). We observe that this ceases to be true in strategic classification --- there are examples where randomized linear classifiers can achieve strictly better accuracy than any deterministic linear classifier (similar result is observed by Braverman and Garg \cite{braverman2020role}; see related work for more discussion). Interestingly, however, we prove that randomization does \emph{not} improve accuracy for   classification with evasion adversaries, by leveraging the special properties of the cost function in adversarial classification.  



%  We study strategic classification for arguably the most basic 
% classifier hypothesis class---\emph{linear classifiers}. Our contributions are summarized below.
% \begin{itemize}[leftmargin=2mm, noitemsep, topsep=0pt]
% \item 
% We study strategic linear classification with arbitrary rewards and an $\ell_p$ norm cost function---this generalizes both adversarial as well as prior strategic classification results. As a result, our notion of \emph{strategic VC-dimension}, and the corresponding bound, generalizes the corresponding notion for adversarial and non-strategic settings.
% We show that strategic linear classifiers are statistically learnable; however, in general, they are not efficiently learnable.
% \item 
% Perhaps surprisingly, we show that randomization (over linear classifiers) is provably helpful, i.e., strictly increases accuracy over any deterministic classifier in strategic settings. Note that this is not true for non-strategic classification. This also doesn't hold for the separable cost functions considered in~\cite{hardt2016stratclass}. 
% \item 
% We show that randomized strategic classification is also statistically learnable under certain conditions on the rewards, and can be efficiently learned in fixed dimensions; we prove its NP-hardness in general. \anil{we drop this point, right?}
% \end{itemize}

% \hf{In a nutshell, our model can be viewed as a generalization of previous adversarial classification and strategic classification models.  }
% \anil{the ``generalized'' part is not coming out clearly in the intro. Also, since we are making the three points about Hardt et al, we probably need to address it directly}




% In a number of domains, e.g., , individuals are able to modify their attributes
% (at some cost), and affect the outcomes of machine learning methods, often with high stakes.
% This behavior is sometimes referred to as ``gaming'', or , and this is often
% used to keep a classification method secret~\cite{Citron201489WashLRev0001TS}.
% This is not fool-proof, in general, as the methods can be reverse engineered in many settings;
% further, transparency of machine learning methods is sometimes mandated by law, e.g.,~\cite{goodman2016regulations}. Hardt et al.~\cite{hardt2016stratclass} introduced the notion of \emph{strategic classification} motivated by these issues, using a Stackelberg game framework, involving a Jury (who designs a classification scheme, and is interested in ensuring good accuracy),
% and a contestant (who corresponds to the data points, and is interested in altering his/her input features to be classified as a ``$+1$''). There is a cost for changing the input features, and the utility for the contestant is the difference of the reward from getting labeled $+1$ and the cost. When the rewards are all uniform, and the cost of manipulation is ``separable'' (defined in Section~\ref{sec:prelim}), Hardt et al.~\cite{hardt2016stratclass} show how to design classification schemes which are robust to manipulation. Since then, there has been a lot of work in this direction, e.g.,~\cite{hardt2016stratclass, dong:ec18, milli:fat19}.





% For the problem of university admission, the training data are the population of past students. The university has already known very well about those students and thus have their true features, labels and preferences. The university would like to use such historical data to learn a good classifier for future admission decisions. However, any new application (i.e., a test data point) may manipulate his/her features. 
 



\subsection{Additional Discussions on Related Works, and Comparisons}\label{subsec:related}

%{\bf Strategic Classification. } 
Most relevant to our paper is the recent work by Hardt et al. \cite{hardt2016stratclass} who introduced the Stackelberg game framework to model the interaction between the learner and the test data. As mentioned previously, our model can be viewed as a strict generalization of \cite{hardt2016stratclass} by allowing \emph{heterogeneous} preferences over classification outcomes.  Assuming a special class of  \emph{separably cost functions}, \cite{hardt2016stratclass} proves that the optimal classifier,  among all possible binary classifiers,  is always a \emph{threshold} classifier. Therefore, the assumption of separable cost functions essentially reduces the feature space to one dimension. Despite the clean characterization this assumption yields, it appears a strong and somewhat unrealistic requirement. For example, one consequence of  separable cost functions is that  for \emph{any} two features $\x, \z$, the manipulation cost from either $\x$ to $\z$ or from $\z$ to $\x$ must be $0$.\footnote{A cost function $c(\z; \x)$ is separable if there exists two functions $c_1, c_2: \X \to \RR$ such that $c(\z; \x) = \max \{ c_2(\z) - c_1(\x), 0 \}$. Since $c(\x; \x) = 0$, we have $c_2(\x) \leq c_1(\x)$ for any $\x$. Therefore, $c_2(\x) + c_2(\z) - c_1(\x) - c_1(\z) \leq 0$. Consequently, either $c_2(\x)  - c_1(\z) \leq 0$ or $ c_2(\z)- c_1(\x) \leq 0$, yielding either $c(\z; \x) =0$ or $c(\x; \z) =0$.} This is not realistic in reality. For example, a student  with true (average  school grade, SAT score) level as  $(85,1500)$ is likely to incur cost in order to score $(95, 1300)$  and vice versa, because  different students are good at different aspects. Our model imposes less assumptions on the cost functions, except that they are induced by   arbitrary semi-norms. %\todo{need to justify this assumptions by citing other works} 
Working with this broader and more realistic class of cost functions,  we do not have the universal and simple characterization of the optimal classifier any more. This is why we  have to take the classic approach and define learnability for a hypothesis class of classifiers, captured by our novel notion of strategic VC-dimension. As an instantiation of our framework, we then study the efficient learnability, both statistically and computationally, of the ubiquitous linear classifiers. %From this perspective, our insistence on a broader and more realistic class of cost functions necessitate a different set of research questions from \cite{hardt2016stratclass} that we address in this work.  

There has been much recent interest in strategic classification. \cite{bruckner2011stackelberg} is one of the first to consider the Stackelberg game formulation of strategic classification, motivated by spam filtering. They primarily focused on the optimization problem of solving the Stackelberg classification game without deriving  generalization bounds. Zhang and Conitzer \cite{zhangincentive} study PAC learning for strategic classification under incentive-compatibility constraints, i.e.,  subject to no data points will misreport features. These two works all assume the positive labels are always and equally preferred. There has also been work on understanding the social implications of strategically robust classification~\cite{akyol2016price,milli:fat19,hu:fat19}; these works show that improving the learner's performance may lead to increased social burden and unfairness. Dong et al. \cite{dong:ec18} and Chen et al. \cite{chen2020learning} extended strategic linear classification to an online setting where the input features are not known a-priori, but instead are revealed  in an online manner. They both focused on the optimization problem of regret minimization.   Our setting however is in the more canonical PAC-learning setup and our objective is to design statistically and computationally efficient learning algorithms. All these aforementioned works, including the present work,  consider \emph{gaming} behaviors. A relevant but quite different line of recent works study \emph{strategic improvements} where the manipulation does really change the inherent quality and labels \cite{kleinberg2019classifiers,miller2019strategic,ustun2019actionable,bechavod2020causal,pmlr-v119-shavit20a}. The question there is mainly to design  incentive mechanisms to encourage agents' efforts or improvements.  




%Finally, another line of works that has similar flavor to us but is significantly different is  strategic regression \cite{Perote2004StrategyproofEF,dekel2010incentive,chen:ec18}. These are different machine learning problems and moreover, the strategic manipulations considered in these  works are during the training phase whereas ours are during the testing phase.     

% Regression is another basic machine learning questions, which are studied under strategic setups \cite{Perote2004StrategyproofEF,dekel2010incentive,chen:ec18}.  



As mentioned earlier, our model of strategic classification also strictly generalizes the problem of  \emph{adversarial classification with evasion attacks}, which has been studied in numerous applications, particularly deep learning models \cite{biggio:ecml13, biggio:icml12,li2014feature,carlini:sp17, goodfellow2015explaining, Jagielski2018ManipulatingML, moosavi:cvpr17, mozaffari:jbhi15, rubinstein:sigmetrics09}.  Our focus here however is on the theoretical side.  Most relevant to our paper is the recent work by Cullina et al. \cite{cullina:nips18}. They introduced the notion of adversarial VC-dimension, which we generalize in this paper. We also  show the connections and differences between our strategic VC-dimension and AVC. Notably, AVC can be viewed as a special case of SVC. Moreover, we studied computational efficiency as well whereas \cite{cullina:nips18} focuses only on statistical  efficiency of learning. In a different work, Awasthi et al. \cite{awasthi2019robustness}  studied \emph{computationally} efficient learning of linear classifiers under $l_{\infty}$-norm $\delta$-ball adversarial classification. Our computational tractability results can be viewed as a generalization of their results to $\delta$-ball  induced by \emph{arbitrary semi-norms} in adversarial classification.\footnote{Awasthi et al. \cite{awasthi2019robustness} also studied computational tractability of learning other classes of classifiers, e.g., degree-2 polynomial  threshold classifiers.} 

% The above questions are related to the area of adversarial machine learning, which involves studying vulnerabilities due to manipulations in training or test data, e.g.,~\cite{cullina:nips18, biggio:ecml13, biggio:icml12, carlini:sp17, goodfellow2015explaining, Jagielski2018ManipulatingML, moosavi:cvpr17, mozaffari:jbhi15, rubinstein:sigmetrics09, awasthi2019robustness}. However, strategic learning is more complex in a sense, because each data point is manipulated based on its local utility, unlike in adversarial perturbations, and prior results for the adversarial setting are not easily usable for strategic classification.


Our last technical section examines the power and limit of randomization in strategic classification. Braverman and Garg \cite{braverman2020role} recently show that randomized linear classifier can strictly improve strategic classification even in $1$-dimensional feature space, when the cost function is \emph{instance-wise}. Our results complements this finding by proving that when cost function is \emph{instance-invariant}, randomization will not be helpful in $1$-dimensional feature space, but we show it can strictly improve classification accuracy in $2$-dimensional feature space. Moreover, to our knowledge, our result of showing the limit of randomization in adversarial classification is new.         


Finally, going beyond classification, strategic behaviors in machine learning has received significant recent attentions, including in regression problems \cite{Perote2004StrategyproofEF,dekel2010incentive,chen:ec18}, distinguising distributions \cite{zhang2019distinguishing,zhang2019samples}, and learning for pricing \cite{amin2013learning,mohri2015revenue,vanunts2019optimal}. These are similar in spirit to us, but study a completely different set of problems using different techniques. Their results are not comparable to ours. 

% The Jury-Contestant framework for strategic classification was introduced by Hardt et al. \cite{hardt2016stratclass} who assume that all data points always equally prefer $+1$ label.  They considered a special class of cost functions called  separable functions of the form $c(\mathbf{y};\x) = \max \{ 0 , c_2(\mathbf{y}) - c_1(\x) \}$ for some functions $c_1$ and $c_2$. One of the main findings of \cite{hardt2016stratclass} is that with separable cost functions the optimal strategic classifier is efficiently learnable for any function $h$ with bounded Rademacher complexity; in fact, the solution is a simple threshold function. This is possible intuitively because  separable cost functions essentially map any feature space into a one-dimensional feature space; Our Corollary~\ref{cor:hardt} provides some theoretical explanation for this intuition.  There has also been work on understanding the social implications of strategically robust classification~\cite{milli:fat19, hu:fat19}; these show that improving the Jury's performance can lead to increased social burden and unfairness. On the other hand, \cite{kleinberg2019classifiers} shows that carefully designed strategic classifiers can incentive the right effort and thus improves individuals.  Dong et al.~\cite{dong:ec18} extend this to an online setting, where the input features are not known a priori, and have to be learned in an online manner. Going beyond classification, strategic behaviors in machine learning has received significant recent attentions, including in regression problems \cite{DEKEL2010759,chen:ec18} and learning for pricing \cite{amin2013learning,mohri2015revenue,vanunts2019optimal}. These are similar in spirit to us, but study a completely different set of problems using different techniques. Their results are not comparable to ours. 



%connection with adversarial 


==> rand.tex <==
\section{The Power and Limits of Randomization}\label{sec:rand}
It is well-known that in standard classification, randomization over the classifiers cannot result in strictly smaller loss. Interestingly, it turns out that randomization can lead to strictly smaller loss in strategic classification, as we  show in this section.  We start by defining randomized classifiers as follows.

\begin{definition}[Randomized Binary Classifiers] A binary classifier $H$  is called a randomized classifier over \emph{any} hypothesis class $\H$ (not necessarily linear classifiers) if there exists a set of deterministic classifiers $\{h_1,\ldots, h_k\} \subseteq \H$, and a probability vector $\mathbf{p} = \{p_1,\ldots, p_k\}$ with $\sum_j p_j = 1$, such that for any input feature $\x$, $H(\x) = h_j(\x)$ with probability $p_j$.
\end{definition} 

The capital $H$ notation is to distinguish randomized classifiers from deterministic ones, and can be viewed as a random variable. Since we always focus on binary classification,  we simply say randomized classifiers henceforth. Note that randomized classifier should not be confused with classification methods like logistic regression or ensemble methods (e.g., random forest), which ultimately still output a deterministic label. The following proposition, whose proof is deferred to Appendix \ref{append:sec:rand:rand-2D-linear}, shows that randomization can help in strategic linear classification. 
% Overloading the notation, for binary classification we also use $f$ to denote a \emph{randomized classifier}. As a natural generalization, $f$ now maps $\R^d $ to $[0,1]$ where $f(\x)$ is interpreted as the probability that $\x$ is labeled $+$.      


% \noindent 
% \textbf{The Randomized Strategic Classification (\probrand) problem.}
% Given uncontaminated input $(\mathbf{x}_1, y_1), \cdots, (\mathbf{x}_n, r_n)$  drawn i.i.d. from $\D$, the \probdet{} problem involves  finding a set of classifiers $\mathcal{F} = \{f_1,\ldots, f_k\}$, and a probability vector $\mathbf{p} = \{p_1,\ldots, p_k\}$, such $\sum_i p_i = 1$, which minimizes the expected \emph{strategic 0-1 loss}, defined as follows:
% \begin{equation}
%     \text{Strategic 0-1 Loss of }\mathcal{F}: \quad \mathbb{E}[L(\mathcal{F};\D)] = \Pr_{(\x, y, r) \sim \D} \sum_{i=1}^k p_i \cdot \big[ f_i(\Delta(\x,r)) \not = y \big]. 
% \end{equation}

% Under the above strategic behavior, given any classifier $f$, let $SP_+(f) = \{ \mathbf{x}:  f(\Delta(\mathbf{x}) ) = +1\} $ denote the set of points which will be classified as $+1$ after agent's strategic manipulation. That is,  $SP_+(f)$ is the positive region of classifier $f$ under strategic behavior where $P_+(f)$ is the positive region of classifier $f$ under honest behavior.

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/ex5.png}
% \caption{
% One dimensional setting. $a_-$ is the \# of ``-'' in $(L_1, L_1+1/2)$, and so on. $a_+=0$, so there are no ``+'' labels in $(L_1, L_1+1/2)$.
% }
%     \label{fig:1d}
% \end{figure}


% Consider the example of Figure~\ref{fig:1d}. 
% \begin{eqnarray*}
% \mbox{err}(L_1) &=& \#^-(L_1, L_1+1) + \#^+(L_1+1, L_2+1)\\
% \mbox{err}(L_2) &=& \#^-(L_1, L_2+1)\\
% \mbox{err}\Big(\frac{1}{2}L_1 + \frac{1}{2}L_2\Big) &=& \#^-\Big(L_1, L_1+\frac{1}{2}\Big) + \frac{1}{2}\#^+(L_1+1/2, L_2+1/2) + \frac{1}{2}\#^-\Big(L_1+\frac{1}{2}, L_2+\frac{1}{2}\Big) + \#^+\Big(L_2+\frac{1}{2}, L_2+1\Big) 
% \end{eqnarray*}

% For the instance in Figure~\ref{fig:1d}, we have
% \begin{eqnarray*}
% \mbox{err}(L_1) &=& a_- + b_- + c_+ + d_+ = a_- + b_- + c + d\\
% \mbox{err}(L_2) &=& a_- + b_- + c_- + d_- + e_- = a_- + b_- + c + d + e_- \\
% \mbox{err}\Big(\frac{1}{2}L_1 + \frac{1}{2}L_2\Big) &=& a_- + \frac{1}{2}b_- + \frac{1}{2}c_+ + \frac{1}{2}c_- + \frac{1}{2} d_- + \frac{1}{2}d_+ = a_- + \frac{1}{2}b_- + c + d
% \end{eqnarray*}

% Therefore, if $b_- >0$ and $d>0$, we have $\mbox{err}\Big(\frac{1}{2}L_1 + \frac{1}{2}L_2\Big) < \min\{\mbox{err}(L_1), \mbox{err}(L_2)\}$. Other possible deterministic classifiers also have higher error:

% \begin{eqnarray*}
% \mbox{err}(L_1 + 1/2) &=& a_- + b_- + c_+ + d_+\\
% \mbox{err}(L_1+1) &=& a_- + b_- + c_+ + d_+\\
% \mbox{err}(L_2+1/2) &=& a_- + b_- + c_- + d_-
% \end{eqnarray*}





% \subsection{Example for $\ell_{\infty}$ norm}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/ex4.png}
%     \caption{
%     Example for the $\ell_{\infty}$ norm
%     }
%     \label{fig:ell-inf}
% \end{figure}

% In Figure~\ref{fig:ell-inf}, a single line does not work. We consider a random classifier with lines $L_1$ and $L_2$, each picked with probability $1/2$. For node B, the expected utility is $0.5\cdot 2 - 1.1$, so it does not move past line $L_1$. Node A gets utility $2-1.6$ by moving past the intersection point



\begin{proposition}\label{prop:rand-2D-linear}
There are strategic classification instances which are perfectly separable by a \emph{randomized} linear classifier  but not by  any deterministic linear classifier.  This is true even when all data points have the same reward value $r$. 
\end{proposition}




The advantages of randomized classifiers over deterministic classifiers  fundamentally comes from the strategic data points' tradeoff between two factors: (a) manipulation cost; (b) the gain from classification outcomes. Interestingly, \emph{if any of these two factors is absent, then randomization will not be beneficial}. First, if there is no gain from classification outcome (i.e., $r=0$ for any data point), then naturally the data points have no benefit to move and thus will stay put. This is precisely the classic classification setup. Second, our following result shows that if data points have no moving cost, randomization will not help neither in the separable case. Formally, we consider a special type of strategic classification where each data point is constrained to move within a designated region which can be \emph{arbitrary} (even can be unconnected) and has no moving cost, i.e., $c(\z; \x) = 0$ for any feasible move. We term this the \emph{zero-manipulation-cost} strategic classification. Note that the adversarial or robust classification setup falls into this case \cite{cullina:nips18,awasthi2019robustness}. 

\begin{theorem}
\label{thm:rand-no-help}
 Consider \emph{zero-manipulation-cost} strategic classification. For any hypothesis class $\H$, if there is a randomized  classifier over $\H$ that perfectly separates the positive points from the negative (i.e., achieving $0$   loss), then there must exist a deterministic  classifier in $\H$ that achieves so as well. 
\end{theorem}

In adversarial classification, it is usually assumed that each data point can move  within a $\delta$-ball around it with no cost. 
An immediate corollary of Theorem \ref{thm:rand-no-help} is the following. 
\begin{corollary}
Randomization does not help in any perfectly separable adversarial classification problems.  
\end{corollary}

We remark that   perfectly separable assumption in Theorem \ref{thm:rand-no-help} is necessary. That is, even for zero-manipulation-cost strategic classification problem, there are non-separable examples where randomized linear classifier can achieve strictly larger accuracy  than any deterministic linear classifier, as shown in the following proposition with proof deferred to Appendix \ref{append:sec:rand:randhelp}. 
\begin{proposition}\label{prop:randhelp}
%Let $\cH_d$ be the class of binary linear classifiers on $\mathbb{R}^2$, and $\tilde{\cH}$ be the class of randomized binary classifiers over $\cH$. 
There exists zero-manipulation-cost \emph{non-separable} strategic classification instances in $\RR^2$  where the  minimum  risk of any deterministic linear classifier is strictly larger than some randomized linear classifier. 
\end{proposition}


% \begin{proof}
% Assume a classifier $L$ that randomizes over $k$ hyperplanes $l_1, \cdots, l_k$ and achieves zero loss. We claim that any deterministic linear classifier $l_i$  will also achieve zero loss and thus the randomization is not needed.  

% Consider any data point $(\x, r)$.  Let its best move in classifier $L$ to be $\Delta(\x)$. By assumption of zero loss, we know that $l_i$ will classify $\x$ correctly, meaning $l_i(\Delta(x))$ is the true label of $\x$. We argue that if we deterministically deploy $l_i$, it will also classify $\x$ correctly. The only worry here is that $\x$ was originally classified as label $0$ but when only $l_i$ is deployed, $\x$ may want to cross $l_i$ and move to another location $\Delta'(\x)$ to receive label $1$. Recall that this is precisely the case in Figure \ref{fig:RandExample}.  However, this cannot happen when costs are zero. Otherwise, $\x$ could have already moved to $\Delta'(\x)$ to achieve a positive reward when the original randomized classifier $L$ is deployed because there is no cost of such a feasible move. This contradicts the fact that original classifier $L$ is perfect. 

% In fact, the above argument goes through even when the reward $r$ is negative, i.e., $\x$ prefers label $0$ but was correctly classified as label $1$. This is precisely the case for adversarial classification.     
% \end{proof}

% For example, if the  move has no cost but has to be within a small region, one can show that  then randomization would not help. This is precisely the case for adversarial or robust classification where moving cost is 0 as long as moving within radius $\sigma$.   

% Remark 2: we consider loss functions that are additive (and therefore linear) over test points. For such loss functions, in the truthful setting (where points cannot move) there is no benefit to a randomized classifier since the loss of the randomized classifier is a convex combination of the loss over the corresponding deterministic classifiers and so one of the deterministic classifiers must achieve a loss no worse than that of the randomized classifier. However, in the strategic case this is no longer assured as shown by the above example.

% Remark 3: we will need to investigate the landscape of loss functions and metrics to understand how and when randomization helps. 

% Remark 4: It could be interesting to consider transferable utilities where the budget is not point-by-point but a total shared across points. There might also be an interesting Braess paradox like situation where the benefit to a point is dependent on other points so that coordination beats anarchy. 

% The constructed example in Figure \ref{fig:RandExample} is 2-D. One might wonder what happens in one-dimensional situation. Our next proposition shows that randomization does not help for  one-dimensional data features. This is fundamentally due to some order structure of the classifiers in one dimension.

% \begin{proposition}\label{prop:rand-1-D}
% For strategic classification with one-dimensional features and uniform rewards, there is no benefit to the randomized linear classifier over the deterministic ones. 
% \end{proposition}

% \begin{proof}
% Setup: consider the 1-D line running from $-\infty$ on the left to $+\infty$ on the right. There are a lot of $+$'s on the left and a lot of $-$'s on the right. A (discrete) randomized classifier can be seen as a set of ordered points $x_i, 1\leq i \leq n, x_i < x_{i+1}$ with associated probability $p_i$. A deterministic classifier is the special case of a single point x with probability $p_x = 1$.

% The first observation is that the 0-1 loss with a deterministic classifier $x$ in the strategic setting is the same as with the deterministic classifier $x + 1$ in the strategic setting. 

% Easy case (good spacing property): Consider a randomized classifier such that $x_{i+1} - x_i > p_i$; it is easy to see by the above observation that the loss of the classifier is the same as the loss of the randomized classifier $x_i + p_i, 1\leq i \leq n$ in the truthful setting. But in the truthful setting there is a deterministic classifier $x^*$ with loss no worse so if we take the corresponding $x^*-1$ we get a deterministic classifier in the strategic setting that is at least as good.

% Slightly harder case: suppose we don't have the good spacing property then there must be two points in the support, $x < y$ such that $x + p_x > y$, but in this case observe that any minus point in $[x, x + p_x + p+q]$ would move to the left of $x$ and hence the error of the classifier would be no worse if we dropped the point $y$ and increased the probability of $x$ to $P_x + p_y$. 

% \end{proof}


%\hf{This proof might not work if $r_i$s are different for different data points....}
% \begin{proof}
% Setup: consider the 1-D line running from $-\infty$ on the left to $+\infty$ on the right. There are a lot of $+$'s on the left and a lot of $-$'s on the right. A (discrete) randomized classifier can be seen as a set of ordered points $x_i, 1\leq i \leq n, x_i < x_{i+1}$ with associated probability $p_i$. A deterministic classifier is the special case of a single point x with probability $p_x = 1$.

% The first observation is that the 0-1 loss with a deterministic classifier $x$ in the strategic setting is the same as with the deterministic classifier $x + 1$ in the strategic setting. 

% Easy case (good spacing property): Consider a randomized classifier such that $x_{i+1} - x_i > p_i$; it is easy to see by the above observation that the loss of the classifier is the same as the loss of the randomized classifier $x_i + p_i, 1\leq i \leq n$ in the truthful setting. But in the truthful setting there is a deterministic classifier $x^*$ with loss no worse so if we take the corresponding $x^*-1$ we get a deterministic classifier in the strategic setting that is at least as good.

% Slightly harder case: suppose we don't have the good spacing property then there must be two points in the support, $x < y$ such that $x + p_x > y$, but in this case observe that any minus point in $[x, x + p_x + p+q]$ would move to the left of $x$ and hence the error of the classifier would be no worse if we dropped the point $y$ and increased the probability of $x$ to $P_x + p_y$. 

% \end{proof}





% \begin{proof}
% The proof follows exactly the same argument as that of Proposition \ref{prop:rand-1-D} by arguing in the space of $c_2(\y)$.  
% % We argue that the classification problem is equivalent to the following one-dimension classification problem. For each data point $(\x, r)$, we construct  a new one-dimensional data point with feature value $c_1(\x)$ and reward $r$. The cost function is defined as $\max \{ 0, c_2(\y) - c_1(\x) \}$. The classification is equivalent tot this one dimensional classification problem. 
% \end{proof}


